Development of a Simulation Model and Precise Timing Techniques for PICOSEC-Micromegas Detectors

This work aims at the development of signal processing algorithms that can explore the potential of a PICOSEC-MicroMegas detector and offers the ability for online, precise timing. The PICOSEC-MicroMegas detector is a novel gaseous detector offering precise timing resolution in experimental measurements. The performance of the proposed signal processing algorithms is evaluated by a variety of tests using experimental data. The data used in the present research were accumulated during a Laser Beam Test at CEA/IRAMIS-SACLAY. We use two sets of experimental events: the SPE-set comprises single photoelectron waveforms, and the EXP-set contains waveforms corresponding to an average of 7.8 photoelectrons. The EXP-set waveforms, when fully analyzed, resulting in a timing resolution of 18.3 $\pm$ \,0.2 ps. Alternative algorithms, based on Constant Threshold Discrimination, but using multi-Charge above the threshold to correct for systematic timing effects, are described and evaluated in detail. Furthermore, a timing technique using Artificial Neural Networks(ANN) has been advanced and evaluated. To generate appropriate learning set for the ANN, a novel simulation model has been developed. We have used the EXP-set waveforms, to quantify the accuracy of the developed techniques and we found that the same timing precision, as in the full signal processing analysis, is achieved. We have also proved that the estimation of the Signal Arrival Time using the developed techniques is consistent and unbiased. Finally, another attractive feature of the newly developed techniques is the fact that they can be used during data acquisition to provide fast timing of the arrival of the particles for triggering and event selection.

==> chapters/ANN.tex <==
\vspace{-0.8cm}
\noindent\fbox{%
    \parbox{\textwidth}{ Later on in this chapter, a simulation model is being represented, as a prerequisite for developing an Artificial Neural Network timing technique. 
    }%
}


==> chapters/abbreviations.tex <==
% \newpage
%     \begin{center}
    
%         \vspace*{0.1cm}
%         \Large
%         {Nomenclature}\\
%         \vspace{0.5cm}
        
%     \end{center}

% \begin{tabular}{ l l }
%  BMS & Battery Management System \\ 
%  isoSPI & Isolated SPI communication \\
%  OCV & Open-Circuit Voltage\\
%  PEC & Packet Error Code\\
%  HV	& High Voltage\\
%  LV	& Low Voltage\\
%  SAE & Society of Automotive Engineers\\
%  AUTOSAR & AUTomotive Open System ARchitecture\\
%  VCU & Vehicle Control Unit\\
%  ECU & Electronic Control Unit\\
%  EMI & Electromagnetic Interference\\
%  RWD & Rear Wheel Drive\\
%  LCS & Launch Control System\\
%  TCS & Traction Control System\\
%  PMSM & Permanent-Magnet Synchronous Motor\\
%  CAN & Controller Area Network\\
%  SPI & Serial Peripheral interface\\
%  UART & Universal Asynchronous Receiver/Transmitter\\
%  GPS & Global Positioning System\\
%  IMU & Inertial Measurement Unit\\
%  EKF & Extended Kalman Filter\\
%  PCB & Printed Circuit Board\\
%  DOF & Degree of Freedom\\
%  PID & Partial Integral Derivative \\
%  DAQ & Data Acquisition \\
%  LCD & Liquid Crystal Display \\
%  GUI & Graphical User Interface \\
% \end{tabular}

\mbox{}

\nomenclature{XYZ}{xxx yyy zzz}


\printnomenclature

==> chapters/certificate.tex <==
% \begin{certi}

    \begin{center}
    
        \vspace*{0.1cm}
        \large
        \textbf{K.J. Somaiya College of Engineering, Mumbai-77}\\
        \normalsize
        (Autonomous College Affiliated to University of Mumbai)\\
        
        \vspace{0.8cm}
        
        \large
        \textbf{Certificate}\\
        \vspace{0.5cm}
        
    \end{center}
% \end{certi}
\noindent
{\large This is to certify that the dissertation report entitled \textbf{*insert project name*} submitted by Author Name and Co-author Name at the end of semester VIII of LY B. Tech is a bona fide record for partial fulfillment of requirements for the degree of Bachelors of Technology in Electronics Engineering of University of Mumbai.}
\vspace{2cm}

\begin{table}[h]
\centering
\begin{tabular}{Y Y Y}
\hrulefill & & \hrulefill \\
\large Guide & & \large Head of Department \\
\end{tabular}
\end{table}

\vspace{2cm}

\begin{table}[h]
\centering
\begin{tabular}{Y Y Y}
\hrulefill & & \\
\large Principal & & \\
\end{tabular}
\end{table}

\vspace{1cm}
\noindent
{\large Date:}\\
{\large Place: Mumbai-77}



==> chapters/declaration.tex <==
% \begin{certi}
\newpage
    \begin{center}
    
        \vspace*{-1cm}
        \large
        \textbf{K.J. Somaiya College of Engineering, Mumbai-77}\\
        \normalsize
        (Autonomous College Affiliated to University of Mumbai)\\
        
        \vspace{0.8cm}
        
        \large
        \textbf{DECLARATION}\\
        \vspace{0.5cm}
        
    \end{center}
% \end{certi}
\noindent
{We declare that this written thesis submission represents the work done based on our and / or others’ ideas with adequately cited and referenced the original source. We also declare that we have adhered to all principles of intellectual property, academic honesty and integrity as we have not misinterpreted or fabricated or falsified any idea/data/fact/source/original work/matter in my submission. \par

We understand that any violation of the above will be cause for disciplinary action by the college and may evoke the penal action from the sources which have not been properly cited or from whom proper permission is not sought.}

\begin{table}[h]
\centering
\begin{tabular}{| X | X |}
\hline
 & \\
 & \\
\hrulefill & \hrulefill \\
\textbf{Signature of the Student} & \textbf{Signature of the Student} \\
\vspace{4cm} & \vspace{4cm} \\
 & \\
\textbf{1712XXX} & \textbf{1712XXX} \\
\hrulefill & \hrulefill \\
\textbf{Roll No.} & \textbf{Roll No.} \\
\hline
 & \\
 & \\

\textbf{Signature of the Student} & \\
\vspace{4cm} & \\
 & \\
\textbf{1712XXX} &  \\
\hrulefill &  \\
\textbf{Roll No.} & \\
\hline
\end{tabular}
\end{table}


\noindent
{\large Date:}\\
{\large Place: Mumbai-77}


==> chapters/results.tex <==
\vspace{-0.8cm}
\noindent\fbox{%
    \parbox{\textwidth}{%
        This chapter presents ...
        \\
        \\
    }%
}

\section{Section 1}
Some text ...

\subsection{Sub-section 1}
Some text ...

\subsection{Sub-section 2}
Some text ...
